Planning for an Efficient Implementation of Hypothetical Bousi~Prolog

This paper explores the integration of hypothetical reasoning into an efficient implementation of the fuzzy logic language Bousi~Prolog. To this end, we first analyse what would be expected from a logic inference system, equipped with what is called embedded implication, to model solving goals with respect to assumptions. We start with a propositional system and incrementally build more complex systems and implementations to satisfy the requirements imposed by a system like Bousi~Prolog. Finally, we propose an inference system, operational semantics, and the translation function to generate efficient Prolog programs from Bousi~Prolog programs.

==> test_data_swi_classic.tex <==
       \hline
       \multirow{4}{*}{\textit{\textit{deriv}}}
       & \textsf{Meta1}  & 1.989 & 0.245 & 10,230,177 \\
       & \textsf{Meta2}  & 1.205 & 0.128 & 4,070,102 \\
       & \textsf{Comp}   & 0.491 & 0.030 & 660,078 \\
       & \textsf{Prolog} & 0.491 & 0.023 & 660,077 \\
       \hline
       \multirow{4}{*}{\textit{\textit{fact}}}
       & \textsf{Meta1}  & 2.470 & 0.497 & 11,005,602 \\
       & \textsf{Meta2}  & 1.194 & 0.123 & 4,070,102 \\
       & \textsf{Comp}   & 0.848 & 0.253 & 1,500,077 \\
       & \textsf{Prolog} & 0.888 & 0.231 & 1,500,076 \\
       \hline
       \multirow{4}{*}{\textit{\textit{facttr}}}
       & \textsf{Meta1}  & 2.636 & 0.648 & 11,016,606 \\
       & \textsf{Meta2}  & 1.234 & 0.123 & 4,070,102 \\
       & \textsf{Comp}   & 0.414 & 0.036 & 2,001,077 \\
       & \textsf{Prolog} & 0.450 & 0.056 & 2,001,076 \\
       \hline
       \multirow{4}{*}{\textit{\textit{fib}}}
       & \textsf{Meta1}  & 1.156 & 0.439 & 4,827,118 \\
       & \textsf{Meta2}  & 0.859 & 0.345 & 4,006,022 \\
       & \textsf{Comp}   & 0.109 & 0.006 & 485,645 \\
       & \textsf{Prolog} & 0.111 & 0.002 & 485,644 \\
       \hline
       \multirow{4}{*}{\textit{\textit{nrev}}}
       & \textsf{Meta1}  & 2.258 & 0.575 & 5,699,379 \\
       & \textsf{Meta2}  & 1.194 & 0.127 & 4,070,102 \\
       & \textsf{Comp}   & 0.527 & 0.092 & 1,130,321 \\
       & \textsf{Prolog} & 0.114 & 0.017 & 1,130,320 \\
       \hline
       \multirow{4}{*}{\textit{\textit{path}}}
       & \textsf{Meta1}  & 572.533 & 0.428 & 5,414,424,890 \\
       & \textsf{Meta2}  & 1.197 & 0.130 & 4,070,102 \\
       & \textsf{Comp}   & 0.152 & 0.014 & 1,799,669 \\
       & \textsf{Prolog} & 0.148 & 0.007 & 1,799,668 \\
       \hline
       \multirow{4}{*}{\textit{\textit{primes}}}
       & \textsf{Meta1}  & 4.503 & 0.859 & 29,145,106 \\
       & \textsf{Meta2}  & 1.220 & 0.116 & 4,070,102 \\
       & \textsf{Comp}   & 0.409 & 0.023 & 1,873,577 \\
       & \textsf{Prolog} & 0.408 & 0.016 & 1,873,576 \\
       \hline
       \multirow{4}{*}{\textit{\textit{qsort}}}
       & \textsf{Meta1}  & 2.083 & 0.439 & 10,075,127 \\
       & \textsf{Meta2}  & 1.167 & 0.119 & 4,070,506 \\
       & \textsf{Comp}   & 0.287 & 0.016 & 1,005,071 \\
       & \textsf{Prolog} & 0.256 & 0.008 & 1,005,070 \\
       \hline
       \multirow{4}{*}{\textit{\textit{queens}}}
       & \textsf{Meta1}  & 6.231 & 0.000 & 47,984,882 \\
       & \textsf{Meta2}  & 1.173 & 0.116 & 4,070,102 \\
       & \textsf{Comp}   & 0.417 & 0.000 & 1,971,077 \\
       & \textsf{Prolog} & 0.289 & 0.000 & 1,971,076 \\


==> test_data_swi_hypo.tex <==
       \hline
       \multirow{3}{*}{\textit{\textit{hderiv}}}
       & \textsf{Meta1}  & 2.084 & 0.175 & 11,430,623 \\
       & \textsf{Meta2}  & 1.181 & 0.117 & 4,070,102 \\
       & \textsf{Comp}   & 0.303 & 0.020 & 660,124 \\
       \hline
       \multirow{3}{*}{\textit{\textit{hfact}}}
       & \textsf{Meta1}  & 2.706 & 0.512 & 12,034,102 \\
       & \textsf{Meta2}  & 1.211 & 0.111 & 4,070,102 \\
       & \textsf{Comp}   & 0.703 & 0.077 & 3,012,069 \\
       \hline
       \multirow{3}{*}{\textit{\textit{hfacttr}}}
       & \textsf{Meta1}  & 3.469 & 0.328 & 12,058,106 \\
       & \textsf{Meta2}  & 1.216 & 0.130 & 4,070,102 \\
       & \textsf{Comp}   & 0.670 & 0.044 & 3,514,569 \\
       \hline
       \multirow{3}{*}{\textit{\textit{hnrev}}}
       & \textsf{Meta1}  & 2.742 & 0.386 & 5,699,425 \\
       & \textsf{Meta2}  & 1.164 & 0.119 & 4,070,102 \\
       & \textsf{Comp}   & 0.605 & 0.098 & 1,130,333 \\
       \hline
       \multirow{3}{*}{\textit{\textit{hpath}}}
       & \textsf{Meta1}  & 9.698 & 0.089 & 76,637,002 \\
       & \textsf{Meta2}  & 1.189 & 0.120 & 4,070,102 \\
       & \textsf{Comp}   & 1.330 & 0.102 & 4,537,562 \\
       \hline
       \multirow{3}{*}{\textit{\textit{hprimes}}}
       & \textsf{Meta1}  & 4.694 & 0.277 & 30,589,606 \\
       & \textsf{Meta2}  & 1.241 & 0.119 & 4,070,102 \\
       & \textsf{Comp}   & 0.892 & 0.030 & 5,264,319 \\
       \hline
       \multirow{3}{*}{\textit{\textit{hqsort}}}
       & \textsf{Meta1}  & 2.020 & 0.294 & 10,075,159 \\
       & \textsf{Meta2}  & 1.172 & 0.116 & 4,070,102 \\
       & \textsf{Comp}   & 0.272 & 0.014 & 1,005,083 \\
       \hline
       \multirow{3}{*}{\textit{\textit{hqueens}}}
       & \textsf{Meta1}  & 6.039 & 0.000 & 51,927,280 \\
       & \textsf{Meta2}  & 1.139 & 0.116 & 4,070,102 \\
       & \textsf{Comp}   & 0.289 & 0.000 & 1,971,081 \\
       \hline
       \multirow{3}{*}{\textit{\textit{hypo1}}}
       & \textsf{Meta1}  & 0.700 & 0.017 & 9,090,603 \\
       & \textsf{Meta2}  & 0.042 & 0.004 & 166,743 \\
       & \textsf{Comp}   & 0.939 & 0.162 & 2,023,076 \\
       \hline
       \multirow{3}{*}{\textit{\textit{hypo2}}}
       & \textsf{Meta1}  & 2.045 & 0.081 & 31,618,620 \\
       & \textsf{Meta2}  & 1.498 & 0.128 & 22,657,550 \\
       & \textsf{Comp}   & 1.014 & 0.002 & 4,534,580 \\
       \hline
       \multirow{3}{*}{\textit{\textit{hypo3}}}
       & \textsf{Meta1}  & 1.477 & 0.058 & 22,543,610 \\
       & \textsf{Meta2}  & 1.828 & 0.177 & 22,573,604 \\
       & \textsf{Comp}   & 1.611 & 0.077 & 4,531,578 \\

